Query Circuits: Explaining How Language Models Answer User Prompts

Explaining why a language model produces a particular output requires local, input-level explanations. Existing methods uncover global capability circuits (e.g., indirect object identification), but not why the model answers a specific input query in a particular way. We introduce query circuits, which directly trace the information flow inside a model that maps a specific input to the output. Unlike surrogate-based approaches (e.g., sparse autoencoders), query circuits are identified within the model itself, resulting in more faithful and computationally accessible explanations. To make query circuits practical, we address two challenges. First, we introduce Normalized Deviation Faithfulness (NDF), a robust metric to evaluate how well a discovered circuit recovers the model's decision for a specific input, and is broadly applicable to circuit discovery beyond our setting. Second, we develop sampling-based methods to efficiently identify circuits that are sparse yet faithfully describe the model's behavior. Across benchmarks (IOI, arithmetic, MMLU, and ARC), we find that there exist extremely sparse query circuits within the model that can recover much of its performance on single queries. For example, a circuit covering only 1.3% of model connections can recover about 60% of performance on an MMLU questions. Overall, query circuits provide a step towards faithful, scalable explanations of how language models process individual inputs. The project page is at https://tony10101105.github.io/query-circuit/.

==> algorithms/bon-csm.tex <==
% \begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-2em}
% \begin{minipage}{\linewidth} % keep algorithm boxed
%     \begin{algorithm}[H]
%         \caption{BoN-CSM}
%         \textbf{Input: } Circuits (edge sets) $\{E_1, \dots, E_k\}$ with size in ascending order.\\
%         \textbf{Output: } Score matrix $S$ and tier matrix $T$
%         \begin{algorithmic}[1]
%             \State Initialize $S$, $T$, and boolean matrix $B$.
%             \For{$i, E_i$ in enumerate($\{E_1, \dots, E_k\}$)}
%                 \For{$e$ in $E_i$}
%                     \State $a_e \coloneqq$ attribution score of $e$.
%                     \State $(j, k) \coloneqq$ matrix index of $e$.
%                     \If{$B(j, k)$ is not \textit{True}}
%                         \State $S(j, k) \gets a_e$.
%                         \State $T(j, k) \gets i$.
%                         \State $B(j, k) \gets$ \textit{True}.
%                     \EndIf
%                 \EndFor
%             \EndFor
%             \State \textbf{return} $S$ and $T$
%         \end{algorithmic}
%         \label{alg: bon-csm}
%     \end{algorithm}
% \end{minipage}
% \vspace{-3em}
% \end{wrapfigure}

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-2em}
\begin{minipage}{\linewidth}

\captionof{figure}{BoN-CSM}
\label{alg:bon-csm}

\begin{algorithmic}[1]
  \INPUT Circuits (edge sets) $\{E_1, \dots, E_k\}$ with size in ascending order.\\
  \OUTPUT Score matrix $S$ and tier matrix $T$.

  \STATE Initialize $S$, $T$, and boolean matrix $B$.
  \FOR{$i, E_i$ in enumerate($\{E_1, \dots, E_k\}$)}
    \FOR{$e$ in $E_i$}
      \STATE $a_e \coloneqq$ attribution score of $e$.
      \STATE $(j, k) \coloneqq$ matrix index of $e$.
      \IF{$B(j, k)$ is not \algorithmictrue}
        \STATE $S(j, k) \gets a_e$.
        \STATE $T(j, k) \gets i$.
        \STATE $B(j, k) \gets \algorithmictrue$.
      \ENDIF
    \ENDFOR
  \ENDFOR
  \STATE \textbf{return} $S$ and $T$.
\end{algorithmic}

\end{minipage}
\vspace{-3em}
\end{wrapfigure}


==> algorithms/ibon.tex <==
% \begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-2em}
% \begin{minipage}{\linewidth}  % keep everything boxed
%     \begin{algorithm}[H]
%         \caption{iBoN}
%         \textbf{Input: } Circuits (edge sets) $\{E_1, \dots, E_k\}$ with size in ascending order and edge number constraint $N$.\\
%         \textbf{Output: } An edge set (circuit) $E$
%         \begin{algorithmic}[1]
%             \State Initialize $E$ as an empty edge set.
%             \State Find the largest $i$ s.t. $|E_i| < N$.
%             \State $E \gets E_i$.
%             \State $K \coloneqq N - |E|$.
%             \State $E^{1:K}_{i+1} \coloneqq$ top-$K$ edges of $E_{i+1}$ not in $E_i$.
%             \State $E \gets E \cup E^{1:K}_{i+1}$.
%             \State \textbf{return} $E$
%         \end{algorithmic}
%         \label{alg: ibon}
%     \end{algorithm}
% \end{minipage}
% \vspace{-1em}
% \end{wrapfigure}

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-2em}
\begin{minipage}{\linewidth}

\captionof{figure}{iBoN}
\label{alg:ibon}

\begin{algorithmic}[1]
\INPUT Circuits (edge sets) $\{E_1, \dots, E_k\}$ with size in ascending order and edge number constraint $N$.\\
\OUTPUT An edge set (circuit) $E$.

\STATE Initialize $E$ as an empty edge set.
\STATE Find the largest $i$ such that $|E_i| < N$.
\STATE $E \gets E_i$.
\STATE $K \coloneqq N - |E|$.
\STATE $E^{1:K}_{i+1} \coloneqq$ top-$K$ edges of $E_{i+1}$ not in $E_i$.
\STATE $E \gets E \cup E^{1:K}_{i+1}$.
\STATE \textbf{return} $E$.
\end{algorithmic}

\end{minipage}
\vspace{-1em}
\end{wrapfigure}

